Fundamental Limits of Prompt Compression: A Rate-Distortion Framework for Black-Box Language Models

We formalize the problem of prompt compression for large language models (LLMs) and present a framework to unify token-level prompt compression methods which create hard prompts for black-box models. We derive the distortion-rate function for this setup as a linear program, and provide an efficient algorithm to compute this fundamental limit via the dual of the linear program. Using the distortion-rate function as the baseline, we study the performance of existing compression schemes on a synthetic dataset consisting of prompts generated from a Markov chain, natural language queries, and their respective answers. Our empirical analysis demonstrates the criticality of query-aware prompt compression, where the compressor has knowledge of the downstream task/query for the black-box LLM. We show that there is a large gap between the performance of current prompt compression methods and the optimal strategy, and propose Adaptive QuerySelect, a query-aware, variable-rate adaptation of a prior work to close the gap. We extend our experiments to a small natural language dataset to further confirm our findings on our synthetic dataset.

==> figures/rougeL.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.7\textwidth]{images/rougeL.pdf}
    \caption{Query-agnostic distortion-rate function for the natural language dataset described in \prettyref{app: dataset} using the RougeL metric. Since a higher RougeL metric is better, we plot ``$1 - $ the computed average distortion'').}
    \label{fig: rougeL}
\end{figure}

==> sections/app-limitations.tex <==
% \section{Extension to natural language datasets} \label{app: limitations}

% As discussed in \prettyref{sec: exp_results}, we also use \prettyref{alg: dual-lp} to compute the distortion-rate function for a small natural language dataset.


==> sections/app-query-aware.tex <==

% \section{Extensions to query-aware prompt compression} \label{app: query-aware}


% As mentioned in \prettyref{sec: prompt_comp_RD} and \prettyref{sec: LP_dual}, analogous definitions and results can be obtained for the query-aware setting as well. The difference is that the compressor has access to the query in addition to the prompt. Thus, the compressor $\comp$ is a possibly random function from $\calX \times \calQ$ to $\calM$. For the query $Q$, the compressor maps the prompt $X$ to the compressed prompt $M = \comp(X, Q)$ with $\len(M) \leq \len(X)$. The user provides the input $[M,Q]$ to the LLM, which produces the output distribution $\probP_{\hat Y} = \LLMf{\phi}(M, Q)$. Just as in the query-agnostic setting, two quantities of interest are 
% \begin{center}
%     (1) the (average) {rate} $\bbE\left[\frac{\len(M)}{\len(X)}\right]$,\quad and \quad (2) the {distortion} $\bbE\left[\distlog(Y, \LLMf{\phi}(M,Q))\right]$,
% \end{center}
%  with both expectations taken with respect to the joint distribution $\probP_{MXQY}$.
% Since different queries may require different amounts of information to be preserved during compression, it is also of interest to define the (conditional) rate and distortion \emph{for the specific query $q$} as $\bbE\left[\frac{\len(M)}{\len(X)}\right]$ and $\bbE\left[\distlog(Y, \LLMf{\phi}(M,q))\right]$ respectively, with both expectations taken with respect to the joint distribution $\probP_{MXY|Q}(\cdot | q)$.

% The rate-distortion problem for query-aware prompt compression can be also formulated similarly to \eqref{eqn: RD_prompt_explicit}. We model $\comp$ as a random mapping $\probP_{M|XQ}$ from $\calX \times \calQ$ to $\calM$. Then, the (average) distortion-rate function at rate $R$ is the smallest distortion that can be achieved by a query-aware compressor with rate at most $R$, given by
% \begin{equation}
% \begin{aligned}
% \bar D^*(R) =  \quad \inf_{\probP_{M|XQ}} \quad & \bbE\left[\distlog\big(Y, \LLMf{\phi}(M,Q)\big)\right]\\
% \textrm{s.t.} \quad & \probP_{M|XQ} \text{ is a compressor, and}\\
%             &  \bbE\left[\frac{\len(M)}{\len(X)}\right] \leq R, 
% \end{aligned} \label{eqn: RD_prompt_explicit_conditional_avg}
% \end{equation}
% with both expectations taken with respect to the joint distribution $\probP_{MXQY} = \probP_{M|XQ}\probP_{XQY}$ induced by the compressor. The condition ``$\probP_{M|XQ}$ is a compressor'' is short for (1) for each $x \in \calX$ and $q \in \calQ$, $\sum_{m \in \calM} \probP_{M|XQ}(m|x,q) = 1$, (2) $\probP_{M|XQ}(m|x,q) = 0$ if $\len(m) > \len(x)$, and (3) if $\len(m) = \len(x)$, then $\probP_{M|XQ}(m| x,q) = 0$ unless $m = x$.
% Similarly, the (conditional) distortion-rate function at rate $R$ is the smallest distortion that can be achieved by a query-aware compressor for query $q$ at rate at most $R$, given by
% \begin{equation}
% \begin{aligned}
%  D^*_q(R) =  \quad \inf_{\probP_{M|XQ}(\cdot | \cdot, q)} \quad & \bbE\left[\distlog\big(Y, \LLMf{\phi}(M,Q)\big)\right]\\
% \textrm{s.t.} \quad & \probP_{M|XQ}(\cdot | \cdot, q) \text{ is a compressor, and}\\
%             &  \bbE\left[\frac{\len(M)}{\len(X)}\right] \leq R, 
% \end{aligned} \label{eqn: RD_prompt_explicit_conditional}
% \end{equation}
% with both expectations taken with respect to $\probP_{MXY|Q}(\cdot,\cdot,\cdot|q)$.

% Just like the query-agnostic setting, note that both \eqref{eqn: RD_prompt_explicit_conditional_avg} and \eqref{eqn: RD_prompt_explicit_conditional} are linear programs, as the objective and constraints are all linear in $\probP_{M|XQ}$ and $\probP_{M|XQ}(\cdot | \cdot, q)$ respectively. We obtain explicit linear programs analogous to \eqref{eqn: RD_prompt_LP} by defining constants $\bar \distvec^q_x$ and $\bar \ratevec^q_x \in \bbR_{+}^{\calM_x}$ for the average distortion-rate function and $\distvec^q_x$ and $\ratevec^q_x \in \bbR_{+}^{\calM_x}$ for the conditional distortion-rate functions, for each $x \in \calX$ and $q \in \calQ$, similarly to \eqref{eqn: lp_consts}.


% \begin{proposition}[Query-aware primal LPs] \label{thm: cond-lp} The (average) distortion-rate function for query-aware prompt compression \eqref{eqn: RD_prompt_explicit_conditional_avg} is given by the solution to 
% \begin{equation}
% \begin{aligned}
% \bar D^*(R) =  \quad \inf_{\left(\zvec_{x,q} \in \bbR_{+}^{\calM_x}\right)_{x \in \calX, q\in\calQ}} \quad & \sum_{x \in \calX, q \in \calQ} {\bar{\distvec}}_x^q{}^\top \zvec_{x,q}\\
% \textrm{s.t.} \qquad 
%             &  \sum_{x \in \calX, q \in \calQ} {\bar{\ratevec}}_x^q{}^\top \zvec_{x,q} \leq R,   \\
%             & \mathbf{1}^\top \zvec_{x,q} = 1,  \quad \forall\, x \in \calX,\, q \in \calQ.
% \end{aligned} \label{eqn: RD_prompt_LP_conditional_avg} \tag{avg-cond-LP}
% \end{equation}
% The (conditional) distortion-rate function for query-aware prompt compression for query $q$ \eqref{eqn: RD_prompt_explicit_conditional} is given by the solution to 
% \begin{equation}
% \begin{aligned}
% D^*_q(R) =  \quad \inf_{\left(\zvec_x \in \bbR_{+}^{\calM_x}\right)_{x \in \calX}} \quad & \sum_{x \in \calX} {\distvec^q_x}^\top \zvec_x\\
% \textrm{s.t.} \qquad 
%             &  \sum_{x \in \calX} {\ratevec^q_x}^\top \zvec_x \leq R,   \\
%             & \mathbf{1}^\top \zvec_x = 1,  \quad \forall\, x \in \calX.
% \end{aligned} \label{eqn: RD_prompt_LP_conditional} \tag{cond-LP}
% \end{equation}
% For each $x \in \calX$, $\calM_x$ denotes the set of all possible compressed prompts associated to $x$, i.e., the set of all possible token sequences of length at most $\len(x)$, the vectors $\zvec_{x,q}\in \bbR_+^{\calM_x}$ for $q \in \calQ$ and $\zvec_x\in \bbR_+^{\calM_x}$ are the optimization variables respectively and the constants $\bar \distvec^q_x, \bar \ratevec^q_x, \distvec^q_x, \ratevec^q_x \in \bbR_+^{\calM_x}$ are given by 
% \begin{align}
%     \bar \distvec^q_{x,m} &\triangleq \probP_{XQ}(x,q)\,\bbE \left[\distlog(Y, \LLMf{\phi}(m, q))\right]\enskip\text{and} \enskip
%     \bar \ratevec^q_{x,m} \triangleq \probP_{XQ}(x,q)\,\frac{\len(m)}{\len(x)}, \quad m \in \calM_x, \label{eqn: cond_avg_lp_consts}\\
%     \distvec^q_{x,m} &\triangleq \probP_{X|Q}(x|q)\,\bbE \left[\distlog(Y, \LLMf{\phi}(m, q))\right]\enskip\text{and} \enskip
%     \ratevec^q_{x,m} \triangleq \probP_{X|Q}(x|q)\,\frac{\len(m)}{\len(x)}, \quad m \in \calM_x, \label{eqn: cond_lp_consts}
% \end{align}
% with the expectation taken with respect to $\probP_{Y|MXQ}(\cdot|m,x,q)$.
% \end{proposition}
% \begin{proof}[]
%     This follows immediately from \eqref{eqn: RD_prompt_explicit_conditional_avg} and \eqref{eqn: RD_prompt_explicit_conditional} by defining the constants $\bar \distvec^q_x, \bar \ratevec^q_x, \distvec^q_x, \ratevec^q_x \in \bbR_+^{\calM_x}$ for each $x \in \calX$ and $q \in \calQ$ as given in \eqref{eqn: cond_avg_lp_consts} and \eqref{eqn: cond_lp_consts} and taking $\zvec_{x,q}$ and $\zvec_x$ to be $\probP_{M|XQ}(\cdot | x,q)$ respectively,. We use the fact that $\probP_{M|XQ}(m|x,q) = 0$ when $\len(m) > \len(x)$ to reduce the dimension of $\zvec_{x,q}$ and $\zvec_x$ from $\calM$ to $\calM_x$.
% \end{proof}

% \begin{remark} \label{rmk: variable-rate}
% An interesting phenomenon here that does not occur in the query-agnostic setting is the comparison between the average and conditional distortion-rate functions, i.e., $\bar D^*(R)$ and $D^*_q(R)$ for $q \in \calQ$. One possible way to ``average'' the conditional distortion-rate functions would be to simply compute $\bbE_{Q \sim \probP_Q}\left[D^*_Q(R)\right]$, but we always have $\bar D^*(R) \leq \bbE_{Q \sim \probP_Q}\left[D^*_Q(R)\right]$. This is because the latter averages the distortion-rate functions over $\probP_Q$ at a fixed value of the rate, i.e., the prompt for each query is forced to be compressed to the same rate $R$. For $\bar D^*(R)$, on the other hand, only the \emph{average} rate over the queries is required to be $R$. This allows the compressor to set a higher rate for ``difficult queries'' that have higher distortion values, and use a lower rate for queries that have lower distortion values in general. This is
% exactly the phenomenon we exploit in designing the \emph{variable-rate} compression scheme \aqselect in \prettyref{sec: exp_setup}, which outperforms other existing schemes in our experiments.    
% \end{remark}

% Just as in the query-agnostic setting, it is useful to compute and solve the dual linear programs instead of directly solving the linear programs above.

% \begin{theorem}[Query-aware dual LPs] \label{thm: cond-dual-lp} The (average) distortion-rate function for query-aware prompt compression \eqref{eqn: RD_prompt_explicit_conditional_avg} is given by the solution to the dual of the linear program \eqref{eqn: RD_prompt_LP_conditional_avg}, i.e.,
% \begin{equation}
% \bar D^*(R) =  \sup_{\lambda \geq 0} \left\{ - \lambda R + \sum_{x \in \calX, q\in\calQ} \min_{m \in \calM_x} \left[ \bar \distvec^q_{x,m} + \lambda \bar \ratevec^q_{x,m} \right] \right\}.
%  \label{eqn: RD_prompt_dual_LP_conditional_avg} \tag{avg-cond-dual-LP}
%     \end{equation}
% The (conditional) distortion-rate function for query-aware prompt compression for query $q$ \eqref{eqn: RD_prompt_explicit_conditional} is given by the solution to the dual of the linear program \eqref{eqn: RD_prompt_LP_conditional}, i.e.,
% \begin{equation}
% D^*_q(R) =  \sup_{\lambda \geq 0} \left\{ - \lambda R + \sum_{x \in \calX} \min_{m \in \calM_x} \left[ \distvec^q_{x,m} + \lambda \ratevec^q_{x,m} \right] \right\}.
%  \label{eqn: RD_prompt_dual_LP_conditional} \tag{cond-dual-LP}
%     \end{equation}
% \end{theorem}
% \begin{proof}[] (Conditional) This follows trivially by simply observing that the linear program in \eqref{eqn: RD_prompt_LP_conditional} is identical to that in \eqref{eqn: RD_prompt_LP}, except that $\distvec_x$ and $\ratevec_x$ are replaced by the (conditional) query-aware versions $\distvec^q_x$ and $\ratevec^q_x$ respectively. Henc,  by \prettyref{thm: dual_lp} the solution to \eqref{eqn: RD_prompt_LP_conditional} is given by \eqref{eqn: RD_prompt_dual_LP} with $\distvec_x$ and $\ratevec_x$ replaced by the (conditional) query-aware versions $\distvec^q_x$ and $\ratevec^q_x$ respectively, which gives \eqref{eqn: RD_prompt_dual_LP_conditional}.

% (Average) In addition to replacing $\distvec_x$ and $\ratevec_x$ from \eqref{eqn: RD_prompt_LP} by the (average) query-aware versions $\bar \distvec^q_x$ and $\bar \ratevec^q_x$ respectively, we also have that the optimization variables are given by $z_{x,q}$ for each pair $(x,q)\in \calX \times \calQ$ as opposed to simply $z_x$ for each $x \in \calX$. Hence, by \prettyref{thm: dual_lp} the solution to \eqref{eqn: RD_prompt_LP_conditional_avg} is given by \eqref{eqn: RD_prompt_dual_LP} with $\distvec_x$ and $\ratevec_x$ are replaced by the (average) query-aware versions $\bar \distvec^q_x$ and $\bar \ratevec^q_x$ respectively and $\calX$ replaced by $\calX \times \calQ$. This gives \eqref{eqn: RD_prompt_dual_LP_conditional_avg} exactly, and we are done.
% \end{proof} 

% Note that both \eqref{eqn: RD_prompt_dual_LP_conditional_avg} and \eqref{eqn: RD_prompt_dual_LP_conditional} are of the same form as \eqref{eqn: RD_prompt_dual_LP}, with some minor differences. For a given $q \in \calQ$, the conditional distortion-rate function $D^*_q(R)$ is identical to the query-unaware distortion-rate function $D^*_q(R)$ with $(\distvec_x,\ratevec_x)$ replaced by $(\distvec^q_x, \ratevec^q_x)$, and hence can be solved by running \prettyref{alg: dual-lp} with the input $\left\{R, \left(\distvec^q_x\right)_{x \in \calX}, \left(\ratevec^q_x\right)_{x \in \calX}\right\}$. For the average distortion-rate function $\bar D^*(R)$, in addition to replacing $\distvec_x$ and $\ratevec_x$ by $\bar \distvec^q_x$ and $\bar \ratevec^q_x$, we also have that $\calX$ is replaced by $\calX\times \calQ$, hence $\bar D^*(R)$ is obtained by running \ref{alg: dual-lp} with the input $\left\{R, \left(\distvec^q_{x'}\right)_{x' \in \calX'}, \left(\ratevec^q_{x'}\right)_{x' \in \calX'}\right\}$, where $\calX' \triangleq \calX \times \calQ$ and $x'$ runs over all pairs $(x,q)$.

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

